M3T: A New Benchmark Dataset for Multi-Modal Document-Level Machine Translation

Document translation poses a challenge for Neural Machine Translation (NMT) systems. Most document-level NMT systems rely on meticulously curated sentence-level parallel data, assuming flawless extraction of text from documents along with their precise reading order. These systems also tend to disregard additional visual cues such as the document layout, deeming it irrelevant. However, real-world documents often possess intricate text layouts that defy these assumptions. Extracting information from Optical Character Recognition (OCR) or heuristic rules can result in errors, and the layout (e.g., paragraphs, headers) may convey relationships between distant sections of text. This complexity is particularly evident in widely used PDF documents, which represent information visually. This paper addresses this gap by introducing M3T, a novel benchmark dataset tailored to evaluate NMT systems on the comprehensive task of translating semi-structured documents. This dataset aims to bridge the evaluation gap in document-level NMT systems, acknowledging the challenges posed by rich text layouts in real-world applications.

==> notes.tex <==
title
RAMP: retrieval and style-marking enhanced prompting for style adapted translation

abstract
- a bit wordy, rewrite for clarity and make it more crisp
- leverages in-context learning in large MLMs
- AAT - let's leave it to style adapted translation; otherwise the more generic phrase is "controlled generation"


3.2 Our Approach: RAMP

189: As similarity retrieval requires a relatively larger pool of examples than random retrieval, we leverage cross-lingual prompting to allow a larger number of appropriate examples to be retrieved (see section~\ref{sec:cross-lingual-methods}).

- in Gabriele's experiments there was more diversity across languages because of the IWSLT random split -> source segments were different (~30\%) across languages. If we reverted back to the COCOA-MT data split, then there is not diversity across languages at least for formality - still the case for GenEval-Context

==> packages.tex <==
\usepackage[table,dvipsnames]{xcolor}

\setlength{\belowcaptionskip}{-16pt}

% Remove the "review" option to generate the final version.
% \usepackage[review]{ACL2023}
\usepackage[]{ACL2023}

\usepackage{booktabs,arydshln}
\makeatletter
\def\adl@drawiv#1#2#3{%
        \hskip.5\tabcolsep
        \xleaders#3{#2.5\@tempdimb #1{1}#2.5\@tempdimb}%
                #2\z@ plus1fil minus1fil\relax
        \hskip.5\tabcolsep}
\newcommand{\cdashlinelr}[1]{%
  \noalign{\vskip\aboverulesep
           \global\let\@dashdrawstore\adl@draw
           \global\let\adl@draw\adl@drawiv}
  \cdashline{#1}
  \noalign{\global\let\adl@draw\@dashdrawstore
           \vskip\belowrulesep}}
\makeatother

% Standard package includes
\usepackage{times}
\usepackage{latexsym}

% For proper rendering and hyphenation of words containing Latin characters (including in bib files)
\usepackage[T1]{fontenc}
% For Vietnamese characters
% \usepackage[T5]{fontenc}
% See https://www.latex-project.org/help/documentation/encguide.pdf for other character sets

% This assumes your files are encoded as UTF8
\usepackage[utf8]{inputenc}

% Colored boxes
\usepackage[most]{tcolorbox}

% This is not strictly necessary, and may be commented out,
% but it will improve the layout of the manuscript,
% and will typically save some space.
\usepackage{microtype}

\usepackage{todonotes}
\setuptodonotes{inline}
\usepackage[normalem]{ulem}
\usepackage{array}
\usepackage{wrapfig}

% For subscripting purposes
% \usepackage{fixltx2e}

% For alignment
\usepackage{amsmath}
\usepackage{textgreek}
\usepackage{enumitem,bbding,etoolbox,calc,pifont}

% For references
\usepackage[capitalise]{cleveref}

% This is also not strictly necessary, and may be commented out.
% However, it will improve the aesthetics of text in
% the typewriter font.
\usepackage{inconsolata}

\usepackage{xspace,mfirstuc,tabulary}
\usepackage{pbox}
\usepackage{CJKutf8}

\usepackage[font=small,labelfont=bf]{caption}
\usepackage{multirow}
\usepackage{adjustbox}
\usepackage{amssymb}
\usepackage{bm}
\usepackage[linesnumbered,ruled,vlined]{algorithm2e}
\SetAlFnt{\small}
\SetAlCapFnt{\small}
\SetAlCapNameFnt{\small}
\usepackage{algorithmic}
\algsetup{linenosize=\tiny}

==> sections-long/0-abstract.tex <==
\begin{abstract}

Document translation is problem for neural machine translation (NMT) systems. Most document-level NMT systems are built on top of curated sentence-level parallel data and make the assumption that text from documents and their reading order can be extracted perfectly and that additional visual information (i.e. the document layout) is unimportant. For real-world documents and applications, rich text layouts violate these assumptions – extraction from either optical character recognition (OCR) or heuristic rules can be error prone and layout information (e.g. text blocks, headers, etc.) can convey relations between distant text. This is especially true for PDF documents, a widely used document format that is a visual presentation of document. \bh{Recent advances in modeling...} In this work we introduce a new benchmark dataset to assess systems on the end-to-end task of translating semi-structure documents to address this gap in evaluation document level NMT systems.

% Document translation is problem for neural machine translation (NMT) systems. Most document-level NMT systems are built on top of curated sentence-level parallel data and make the assumption that text from documents, text order in the document can be extracted perfectly and that additional visual information (i.e. the document layout) is unimportant. For real-world documents and applications, rich text layouts violate these assumptions -- extraction from either optical character recognition (OCR) or heuristic rules can be error prone and layout information (e.g. text blocks, headers, etc.) can convey relations between distant text. In this work we introduce a new benchmark dataset to assess systems on the end-to-end task of translating semi-structure documents to address this gap in evaluation document level NMT systems. We introduce a new benchmark dataset to assess systems on the end-to-end task of translating semi-structure documents. We further develop a set of white-box metrics and black-box metrics for assessing translated document quality, taking into account the fidelity of translation. Finally, we investigate the mechanisms through which layout and vision information extracted from pre-trained models (e.g. LayoutLMv2) can be incorporated at training and inference time into existing transformer-based MT models to improve translation quality for structural elements (e.g. titles, bullet points) and to increase robustness to OCR errors.
\end{abstract}

==> sections-long/1-intro.tex <==
\section{Introduction}

\begin{figure*}[th]
    \centering
    \includegraphics[width=\textwidth]{figures/annotations.png}
    \caption{In this work, we introduce a benchmark dataset for PDF document translation. Above from left to right, are example documents sourced from the Eurolex, DocLaynet, and RVL-CDIP datasets demonstrating the complex layout and domains included in the benchmark.  Unlike earlier works, our benchmark focuses on machine translation which depends more heavily on contextual information than earlier works centered around entity extraction.}
    \label{fig:my_label}
\end{figure*}

Traditional machine translation (MT) systems primarily focus on textual content and on a sentence level, ignoring both translations of entire documents and documents that contain visually layouts. While traditional MT systems have made substantial progress in translating individual sentences, their limitations become evident when dealing with documents. Despite advances in segment-level MT that approach human level translation quality [1], a number of recent works have highlighted that there is MT still falls short of human translation quality when whole documents are considered [2,3]. In particular, MT systems generally fail capture inter-sentential context into account, though much recent work however have sought to address this issue through [....cite contextual paper, other contextual works..]

\begin{table}[h]
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{ll}
    \multicolumn{2}{c}{\includegraphics[width=0.75\textwidth]{figures/Example1.png}}  \\ \\
    
    \multicolumn{2}{c}{OCR w/o layout}  \\ \hline
    Src 1 &  general principles for \textbf{implemet-kit} \\
    Src 2 & \textbf{ge comma vocstonal ele poly...} \\ \hline
    Tgt 1 &  allgemeiner Grundsätze für den Implementierungssatz \\
    Tgt 2 & ge Komma Gesang ele Poly... \\
    \hline \hline
    \multicolumn{2}{c}{} \\
    \multicolumn{2}{c}{OCR w/ layout}  \\ \hline
    Src & general principles for implementing  \\
    & a common vocational training policy... \\ \hline
    Tgt & allgemeiner Grundsätze für die Umsetzung  \\
    & einer gemeinsamen Berufsbildungspolitik... 
    \end{tabular}}
    \caption{Examples of errors that occur in a layout-agnostic pipeline translation system. The top image shows the reading order is lost when extracting the text. The downstream translation system cannot recover from such errors resulting in garbled translations. With layout information, the reading order and contiguous blocks of text are preserved, resulting in significantly higher translation usability and quality.}
    \label{layout-aware:examples}
\end{table}

These systems, however, still only treat documents as textual content which ignores much of the visual aspects of documents. For instance, real world documents typically include different typeface in denoting section headings to different parts of the document which indicates to human readers that parts of a document should be treated as a logically distinct. Text blocks can also indicate that sections of text are contextually related and multi-columnar text is easily understood by human readers. Layouts can also indicate that certain text should \textit{not} be translated (e.g. address or name fields) or that tabular data is present. When the layout and visual context is lost, this can result in catastrophic translation errors as we show in Table \ref{layout-aware:examples}.

While recent works have focused on document visual question-answering [4-12], these works have focus on information retrieval tasks where long range contextual clues at the sentence and paragraph level that are needed for MT play less of a role. \xn{[We may demonstrate aforementioned three translation types in a figure: segment-level, contextual, multi-modal.]}

PDF documents, in particular, are a widely used document format that present many of these challenges for modern language models. PDF documents, even those that are digitally borne, can contain artifacts (e.g. white characters on white background to adjust spacing, doubling character placement in cases where bold-face is not available, etc.) that make simple text extraction difficult. They are also visually rich and contain complex layouts where the reading order shifts (e.g. tabular content in a page, multi-columnar data, captions). In this work, we present a multi-modal benchmark dataset for evaluating MT models on translating visually rich PDF documents. With recent advances in multi-modal foundation models \citep{alayrac2022flamingo, openai2023gpt4, liu2023visual, tang-etal-2022-udop}, the ability to benchmark model performance on a challenging document understanding task that takes into account long range contextual clues is of growing importance.

Multi-modal document translation is generally difficult due to the lack of data. One prerequisite for training multi-model document translation is a three-way alignment between source PDF, source text, and target text. \mn{We need some investigation on whether it's required for training. However, it is certainly needed for efficient evaluation.} However, to the best of our knowledge, there are no public parallel datasets that provide the three-way alignment. Finally conventional MT models are  trained and evaluated on sentence-level parallel data. But, the text extracted by from PDF documents may be scrambled, breaking for instance sentence boundaries in the original document or scrambling the sentence order due to changes in reading order of the document. This hinders evaluation and training of such models. \mn{This makes sentence-level evaluation metrics unsuitable for this task}

To bridge this gap in the community, we introduce a new benchmark dataset for multi-modal document translation covering multiple domains, document structure and languages. Furthermore we propose a methodology for generating synthetic three-way aligned training data to enable future research on model development.\footnote{Dataset and scripts can be found here: http://www.github.com/anonymous} To the best of our knowledge, this is the only dataset that combines both document layout and machine translation into a single multi-modal task.  Our contributions are:



\begin{itemize}
    \item[1.] We introduce a new benchmark testset for evaluating end-to-end translation of structured documents (assessing machine translation quality and preserving the layout (textboxes)) \mn{concise description: layout information and reference translations}
    \item[2.] We introduce a black-box metric and white-box metric. 
    \begin{itemize}
        \item The Black-box metric assess end-to-end translation of both digital and image documents (e.g. PDF-PDF)
        \item White-box metric  JSON output (bbox, length preservation, translation) 
        \item human evaluation -> correlation of metric with perceived quality
    \end{itemize}
    \item[3.] We demonstrate the utility of our benchmark on evaluating and analysing the performance of several baseline models
    \begin{itemize}
        \item Pipeline approach - extract, translate using a standard NMT model (regenerate?)
        \item layoutLM style approach - extract, include layout information, translate (train using synthetic data from hyli)
        
        \item layoutLM style approach + multisentence (needs extracting reading order) ((train using synthetic data from hyli)
    \end{itemize}
    
\end{itemize}



==> sections-long/2-related-work.tex <==
\section{Related Work}

Structured document understanding has been a subject of much recent research and in particular intelligent document processing. Much prior work has been focused on information extraction tasks. Inspired by advancements in self-supervised pre-training several works have examined strategies for including multi-modal information (i.e. layout and visual features) in transformer models \citep{Xu2020LayoutLMPO} [5, 6]. [4.5] introduced an additional 2D positional embeddings to make Transformers explicit on layout features. 
Later, [5, 6] improved upon these results by introducing visual features. [15] introduced using visual features of blocks of text while [16] introduced a multi-modal self-attention layer that fused text, visual and layout features. As a whole, these earlier works have been focused on information extraction or text classification tasks. 


Models focused specifically on visually-rich documents
\begin{itemize}
  \item Donut~\citep{kim-etal-2022-donut}: image-only model. Initial work on OCR-free setting.
  \item UDOP~\cite{tang-etal-2022-udop}: multi-modal
\end{itemize}

General vision-language models
\begin{itemize}
  \item PaLI-X~\citep{chen2023palix}: Google's multilngual ~54B parameter vision-language model 
  \item mPLUG-owl2~\citep{}: Alibaba's vision-language model but no explicit support on multiple languages.
\end{itemize}


% where the inputs are image-only 

For generative NLP tasks, like machine translation, performance on visually rich documents has not been explored in as much depth, though others have explored incorporating layout and visual features into machine translation. [13] examined including visual features into machine translation models in order to improve robustness to OCR errors in extracted text, leaving translation at the document level untouched. [17] looked at schema translation of tabular text which .....

In this work, we examine strategies for incorporating multi-modal information for document level translation of visually rich documents. We test the effectiveness of these strategies on a new benchmark a benchmark dataset that includes:


\begin{itemize}
    \item LayoutLM~\citet{Xu2020LayoutLMPO}, XLayoutLM - using layout for information extraction. 
    \begin{itemize}
        \item FUNDS, XFUNDS datasets~\citep{xu-etal-2022-xfund} focus on NER. We have a more challenging dataset
        \item LoRaY - Multilingual dataset focus on text summarization task. We have a parallel dataset suitable for machine translation.
    \end{itemize}
    
    \item Doc2Doc - Documents are taken from WMT-newstest, TED, Europarl - ignores layout information.
    \item Doc2Sent - sliding windows, take from WMT, TED, Europarl - ignores layout
    
\end{itemize}

 Furthermore, we introduce synthetic data generation method that leverages existing parallel data and automatically generated layouts.

==> sections-long/3-method.tex <==
\section{Dataset Description}

Recently, existing sentence-level parallel data have been augmented with paragraph-level, document-level or conversation-level boundaries. While more realistic for evaluating document translation, these datasets are built on the assumption that the text can be extracted from the source document in the correct reading order and without segmentation or word-level errors. In real-word scenarios this is not the case. Translating image or layout rich documents requires both (1) complex, error-prone, text segmentation and extraction methods, as well as (2) adaptation of the translated text to the desired target document layout. Furthermore, translations are influenced by the semantic layout segmentation the text belongs to, for example, a title or a table. 

In this section we introduce a new benchmark, that addresses this gap, consisting of visually-rich documents, annotated with diverse layout elements and with corresponding paragraph-level translations. First, we describe the strategy for sourcing documents with either existing layout annotations or document-level translations. Next, we describe the annotation methodology for creating a parallel data set where both the layout and translations are annotated for multiple languages. Lastly, we introduce a method for synthetic data generation for supervised training of layout-aware document translation models.

\subsection{Data sourcing}


\begin{table}[t]
    \centering
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{l| ccc}
       	& RVL-CDIP & DocLayNet	& Eurolex \\
       	\hline\hline
    Text &	2780 & 6679 & 1325 \\
    Section-header & 144 &	1070 &	999 \\
    Page-footer	& 92 & 685 & 0 \\
    Vertical	& 68 & 133 & 1088 \\
    Table-cell	& 1332	& 16292 & 16451 \\
    Table	    & 44 & 256	& 445\\
    Page-header	& 220 &	525 & 1532 \\
    Picture	& 28 & 444	& 0 \\
    List-item &	204 & 2406 & 1317 \\
    Formula	& 0 & 23 &	2 \\
    Footnote &	0 &	93 & 391 \\
    Code	& 0	& 13 & 0 \\
    Title	& 0	& 74 & 30 \\
    Caption	& 0	& 76 & 24 \\
    \hline \hline
    en-es & 20 & 123 & 54 \\
    en-fr &	20 & 133 & 54 \\
    en-de &	20 & 156 & 54 \\
    en-zh &	20 & 141 & 113 \\
    \hline\hline
    Total & 80 & 553 & 275 \\
    \hline\hline
    Scanned &  80 & -	 & - \\
    Govt. tenders	& - &102 & - \\
    Patents	& - & 36 & - \\
    Legal & - &	71 & 383 \\
    Fin. reports	& - & 344 & - \\
    \hline
    \end{tabular}
    }
    \caption{Distribution of document domains, the layout elements, and language pairs contained in the benchmark dataset. Layout elemnts can be found in Table \ref{annotation:labels}. In the case of Eurolex documents, we used original x$\rightarrow$en documents and produced corresponding english translations so that translations are more likely to fit the original layout elements. In DocLayNet, a mixture of original x$\rightarrow$en and en$\rightarrow$x documents were used. RVL-CDIP documents were originally in english. Finally, RVL-CDIP contains forms and we which were not annotated as a separate layout element.}
    \label{dataset:sampling}
\end{table}


%or  sentences automatically extracted and aligned have traditionally evaluate MT systems on sentence segments with little reference to other aspects of the source document which make them difficult for evaluating multi-modal translation systems. For instance, existing MT document level benchmarks assume text is extracted in the correct reading order (see for example news-commentary, ted) or that there are no errors in the extracted text. 

 We source documents from several existing public datasets that cover a wide range of documents. 
 
 First, we used EUR-Lex\footnote{\url{https://eur-lex.europa.eu/homepage.html}} \xn{Note: It's EUR-Lex, not EuroLex.} to source documents which are translated by professional translators into all the European languages while also preserving the document layout.  These documents are provided in multiple formats, including plain text \citep[XML,][]{steinberger-etal-2006-jrc} and PDF, which allows to automatically extract and align parallel sentences. The resulting sentence-level parallel corpus discards misaligned text and all the layout information. We sample a subset of documents which we annotated with layout information described in the next section. \xn{So the EUR-Lex and JRC-Acquis parallel data generated by Huayang was not used? This internship created a new EUR-Lex dataset by human annotation?}

 Second, we used DocLayNet \cite{doclaynet} and RVL-CDIP \citep{rvl_cdip}, which consist of documents (TODO: domains,types) annotated with layout information. We sourced the documents from their respective test sets to preserve the train/test split that might be used in training layout/vision models (e.g. LayoutLM, X, Y, Z). 

%To test if translation systems generalize to different layout elements, we sampled pages from the test set documents that contained different layout elements. 
For the sampling strategy, we focused on covering a wide range of layout elements.
However, the two layout-annotated datasets did not covered the same subset of layout elements. For these two data sources we sampled for documents containing flat layouts, multi-columnar data, images and tabular information. For Eurolex, we used an initial set of automatically labeled layout elements for sampling documents. We trained the layout classifier using a Faster R-CNN classifier on the DocLayNet dataset using the standard \texttt{dectrctron2} \footnote{https://github.com/facebookresearch/detectron2} following the recommended settings of \citet{doclaynet}. Our classifier reproduced reported results and had an F1 of 73.4 averaged across all layout types. Table \ref{dataset:sampling} reports the distribution of layouts and domain coverage for the sampled documents.

%focused on specific types of documents and did not covered the same set of layout elements, we initially did a but where possible we sampled for elements containing flat layouts, multi-columnar data, images and tabular information. 

\subsection{Document Annotation}

We annotated the sampled documents in two stages. In the first stage, annotators extracted the text and identified and labeled the layout elements. In the second stage, annotators translated the text comprised in each layout element.  

For the layout information, annotators were asked to provide bounding box coordinates and labels for each element. Bounding box labeling means grouping the elements on the page into reasonable paragraphs, headings, tables, pictures, etc. areas on the page, in non-overlapping rectangular areas. For the set of labels, we extended the DocLayNet ontology to include reading order and table cells. Specifically, annotators labelled the layout elements described in Table \ref{annotation:labels}.


\begin{table*}[t]
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l|wwp{0.98\textwidth}}
    Layout & Description \\ \hline
    \textbf{Captions} & Special text outside a picture or table that describes the picture or table. \\ \hline
    \textbf{Footnotes} & Typically small text at the bottom of a page, with a number or symbol that is referred to in the text above. \\ \hline
    \textbf{Formula}& Mathematical equation or chemical formula on its own line. \\ \hline
    \textbf{List-item}& One element of a list, in a hanging shape, i.e., from the second line onwards the paragraph is indented more than the first line. \\ \hline
   \textbf{Page-footer}& Repeating elements like page number at the bottom, outside of the normal text flow. \\ \hline
    \textbf{Page-header}& Repeating elements like page number at the top, outside of the normal text flow. \\ \hline
    \textbf{Picture}& A graphic or photograph. \\ \hline
    \textbf{Section-header}& Any kind of heading in the text, except overall document title. \\ \hline
    \textbf{Table}& Material arranged in a grid alignment with rows and columns, often with separator lines \\ \hline
    \textbf{Table-cell}& Text contained in a cell of a table. \\ \hline
    \textbf{Text-block}& Regular text paragraphs or blocks of text that should be logically grouped together. \\ \hline
    \textbf{Title}& Overall title of a document typically appearing in large font or denoted with special typeface to distinguish it from the rest of the document. \\ \hline
    \textbf{Order}& The order number that the bounding box should be read on the page (i.e. the reading order). For European languages, this is generally left to right, top to bottom. For tables, we adopt a left to right, top to bottom ordering of the cells. \\
    \hline
    \textbf{Vertical} & Text is oriented vertically.\\
    \hline
    \end{tabular}}
    \caption{Layout  elements and their labels annotated in our benchmark following the DocLayNet typology. \mn{If we could move this to the appendix if we show an image of layout annotated document together with Table 1 label statistics.}}
    \label{annotation:labels}
\end{table*}

For translating the extracted text, we provided professional translators with the original document and asked to take into account the context when translating. Extracted text was then translated using a selection of commercial segment level MT systems. Translators were then instructed to post-edit these translations with the additional requirement that the length of the translation within $\pm$10\% of the source text length, which is useful for evaluating how well systems may preserve the original layout of the source document. In order to facilitate length compliance, we sourced documents in de,es, and fr and performed translations into en. For en$\rightarrow$zh we translated from english into chinese.  Table \ref{dataset:sampling}, reports the distribution of layout elements in our dataset. 

 
\subsection{Synthetic data creation}

Fine tuneing, leveraging existing parallel data. there’s a method for creating different layouts and different parallel data. Training data is hard so synthetic data useful. we also do experiments with eurolex. \mn{a lot of work needed here. not sure if we should include this. maybe Xing can help}


\section{Automatic metics}
\mn{are we describing/proposing automatic metrics for this benchmark?}

\mn{Sony might help us with the text-only paragraph-level evaluation}

Figure 1: Example json annotation





==> sections-long/4-experiments.tex <==

% \mn{We could skip this and include comparison with VLMs in the next sections}
% \section{Benchmarking models with our dataset}

% Our primary goal of releasing the multi-modal document translation benchmark is to aid in assessing model performance on a challenging generation task across a variety of layouts and domains. To that end, we evaluated several commerical machine translation system (Amazon, Google, Microsoft ?) and vision-language foundational models. 

% \subsection{Commercial MT systems}
% TODO: translate Docx and PDF using Amazon, Google, Translate. Evaluate translation quality.

% \subsection{Vision-language foundational models}
% TODO: Claude, GPT, LLama ? for document-level translation
% TODO: Flamingo?


\section{Multi-modal document translation}
In this section we further analyse the gaps in translation quality and propose novel multi-modal translation models that address this gap. Specifically, we enhance translation models with information encoded in different modalities: text, layout and image.

\mn{re-organize sections: Baseline, Layout Features, Layout and Vision Features, Experimental Setup, Results, Discussion/Ablation}

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/features_tight.png}
    \caption{We experimented with adding multi-modal features to the embedding space.}
    \label{fig:my_label}
\end{figure}



\subsection{Experimental Methodology}

\subsubsection{Training Data Extraction}
\mn{Xing could you help summarize the block alignemtn strategy implemented by Huayang in 2022}

\subsubsection{Block-level Evaluation}

\subsubsection{Models}

\paragraph{Translation} 
The extracted text is translated using fairseq translation models trained on WMT'19 \cite{wmt-2019} \mn{Huggingface: nllb-200-3.3B}. Throughout the rest of the paper we compare the performance of different systems on translation quality using BLEU scores \footnote{sacrebleu signature}.

\paragraph{Vision and Layout Models}
We used and compared two open-source layout detection models: DocLayNet and Paddle Paddle \mn{todo: citations} (and Tessearct? \footnote{https://github.com/tesseract-ocr/tesseract}). 
\mn{It is not clear which layout models are used for the baseline pipeline and which for extracting embedding features.}


\subsection{Baseline}

In this section we analyse the quality gaps introduced by a baseline layout-agnostic translation system for three language pairs: English $\rightarrow$ German, French, Spanish. A baseline approach is to use an OCR model to extract the text from an image or digital document which is then fed directly to a machine translation model. 

In our experiments, the inputs to the pipeline system are the PDF documents in our benchmark converted to an image format (.jpeg file). To segment and extract text from the input documents we used and compared two open-source layout detection models: DocLayNet and Paddle Paddle \mn{todo: citations} (and Tessearct? \footnote{https://github.com/tesseract-ocr/tesseract}). 

\mn{TODO: explain how we reconstruct alignment between predicted translation and reference by doing source-based alignment of the OCR-ed text}

\subsection{Multi-modal Features}

\paragraph{Layout}

As a first step, we included layout information into the model, and specifically the visual aspects of layout. A common failure mode for translation of OCR'd text is that paragraph level boundaries and especially text divided by visual features in the document, is not well preserved. Headings and paragraphs also tend to be merged together, which lead to errors since sentence boundaries are not properly identified. 

Layout information can exist at different granularity. In our experiments, we tested using the token-level coordinates of bounding boxes typically extracted from OCR tools. \cite{Tapas paper} Next, we added information from a larger visual field that represents text that should be grouped together such as paragraphs, tables and captions. The specific higher-order layout features we considered are the layout group, discrete layout label and the probability of the layout label predicted by the layout model. \mn{TODO: verify features}

Formally, we represent each token $t_{i}$ in a source text snippet by $(e_{t}, x_{0}, y_{0}, x_{1}, y_{1}, l_{cat}, l_{id}, l_{prob})$, the token string, position withing snippet, the bounding box's top-left and bottom-right corners, the layout category, group id and layout label probability. \mn{No width and height?} 

To extract layout features, we trained a vision model on the DocLayNet dataset using a \texttt{detectron2} faster R-CNN model. PDFs were initially converted into images which were then segmented using the faster R-CNN model. The text bounding boxes generated with the vision model were then used to match text found by the OCR model. We used the coordinates and labels of the bounding boxes as layout features for the downstream translation model. Finally, we also tested whether soft predicted layout labels were more useful than hard layout labels and conducted ablation studies using the output probabilities for the layout labels. \mn{this last sentence needs rewriting}

\paragraph{Vision}

Another question we explored is whether visual features are helpful in document translation. Common errors in OCR text generation occur when the quality of the text is not high enough for the model to predict characters, e.g. common errors are ``l$\leftrightarrow$1'', tablular information, listed items, all caps subheadings, etc.  To that end we, we explored including visual features into our model. As a first experiment, we explored adding visual features on the word level which we hypothesize would aid the model in correcting character level errors. Finally since translation is sensitive to longer range dependencies, we also explored adding visual features at the text block level. Visual features were \bh{Talk about linear function to map visual to same dimension.} \mn{details on fine-tuning: how big is the training data, where did we get the training data, did we update all the parameters or only the additional embeddings,add hyperparameters like number of iterations in the appendix.}

\subsection{Results}
\paragraph{Layout-aware Translation}

\begin{table}[h]
    \centering
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{l|cc|cc|cc|}
        & \multicolumn{2}{c|}{En$\rightarrow$De} & \multicolumn{2}{c|}{En$\rightarrow$Fr} &  \multicolumn{2}{c|}{En$\rightarrow$Es} \\
    \textbf{Layout} \rightarrow  &\ding{55}  & \ding{51}  & \ding{55}  & \ding{51}  & \ding{55}  & \ding{51}  \\ % using pifont package for checkmarks
    \hline
    Gnd truth & \multicolumn{2}{c|}{38.4} &  \multicolumn{2}{c|}{36.2} & 
    \multicolumn{2}{c|}{38.3} \\
    \cdashline{1-7}
    Tesseract & 21.2 & 34.1 & 26.8 & 34.1 & 27.4 & 35.7 \\
    System \textract & 23.8 & 33.4 & 22.4 & 32.7 & 22.1 & 34.2 \\
    System \google & \\
    \hline
    \end{tabular}}
    \caption{Evaluation of systems that use layout information to extract and translate continuous blocks of text. BLEU scores are reported on Eurolex testset. The ground truth scores are computed for the system translations of the original source sentences.}
    \label{layout-aware:eurlex:BLEU}
\end{table}



\mn{TODO: explain we added the embeddings of the layout features to the word and positional embeddings.} We found that layout information provides more context and makes translation more robust against OCR errors.

First, we evaluated the baseline pipeline systems that use layout information to extract and translate continuous blocks of text. Results in Table \ref{layout-aware:eurlex:BLEU} show that using layout segmentation improves translation quality in the range of 8 to 13 BLEU points compared to using the OCR text extraction. Still, the quality gap between the best performing pipeline system and the system translating the ground truth text is large, ranging between 2 to 4 BLEU points. \mn{summarize results better}


Table \ref{layout-aware:examples} gives translation examples where we show issues with layout-agnostic systems.




\paragraph{Vision and Layout-aware Translation}

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/textbox_clip.png}
    \caption{Example of visual features: token and block-level image clips.}
    \label{fig:my_label}
\end{figure}



The results in Table \ref{vision-aware-ablation:eurlex:BLEU} that both types of visual features, token and block-level image clips, improve translation quality. However, we the improvements are larger when the training and test data match (Eurolex). We analyse these results by breaking down the scores per layout label \mn{TODO ?} and observe X,Y, Z \mn{are the layouts in the additional dataset not reperesented in Eurolex, e.g. Tables?}. 

\begin{table}[h]
    \centering
    \resizebox{.8\columnwidth}{!}{
    \begin{tabular}{l|c|c|}
        & Eurolex & Additional \\
        \hline
    Gnd. Truth & 32.4 & 42.7 \\
    Tokens Only & 21.7 & 27.1 \\
    \cdashline{1-3}
    Image clip &  25.2 & 28.4 \\
    Image + layout clip & 29.2 & 28.7 \\
    \hline
    \end{tabular}}
    \caption{Ablation of visual features for En$\rightarrow$De document translation quality for a model trained on Eurolex data and evaluated on the Eurolex sourced portion of our dataset and additional documents. We report BLEU scores here. Gnd. truth evaluated utilized ground truth extracted text in the evaluation while tokens evaluated translation using extract tokens using OCR (Tesseract).}
    \label{vision-aware-ablation:eurlex:BLEU}
\end{table}

\subsection{Synthetic data}


Training on synthetic data. important since real labelled data is hard to get. 

\subsection{Ablations}

Finally, we also conducted ablations on whether additional features such as the layout category or image clips are indeed helpful for model performance. To test this, we examined the layout features and image feautres separately. For each, we ablated out model by replacing features randomly and observing the corresponding effect on performance. \mn{In previous sections we only looked and EN-DE. Here we should look at all language pairs.}

\begin{table}[h]
    \centering
    \resizebox{.6\columnwidth}{!}{
    \begin{tabular}{l|c|}
        & Eurolex \\
        \hline
    Gnd. Truth & 36.5 \\
    Tokens Only & 33.1 \\
    \cdashline{1-2}
    Image + layout clip & 35.2 \\
    -- random & -0.5 \\
    Layout + label & 34.1 \\
    -- random & -0.9 \\
    \hline
    \end{tabular}}
    \caption{\mn{The numbers for gnd truth and tokens only don't match the numbers in table 4. Is this a different Eurolex testset?}}
    \label{layout-vision-ablation:eurlex:BLEU}
\end{table}

==> sections-long/5-analysis-ablation.tex <==
\section{Analysis}


==> sections-long/6-conclusion.tex <==
\section{Conclusions}


==> sections-long/7-limitations-impact.tex <==
\section{Limitations}


==> sections/2-related-work.tex <==
\section{Related Work}

Recent research has dedicated considerable attention to understanding structured documents, particularly in the domain of intelligent document processing. Prior efforts have predominantly centered on tasks involving information extraction. In such tasks, most methodologies heavily rely on multi-modal information (such as OCR, layout, and visual features) as inputs to a transformer model \citep{Xu2020LayoutLMPO, xu2020layoutlmv2,huang2022layoutlmv3, tang-etal-2022-udop}. However, the layout merely represents the 2D word bounding boxes extracted from standard OCR systems, and the OCR's reading order typically follows a simplistic raster scan or maximum lines approach concerning the words. 

% Later, [5, 6] improved upon these results by introducing visual features. [15] introduced using visual features of blocks of text while [16] introduced a multi-modal self-attention layer that fused text, visual and layout features. As a whole, these earlier works have been focused on information extraction or text classification tasks. Models focused specifically on visually-rich documents (1) Donut~\citep{kim-etal-2022-donut}: image-only model. Initial work on OCR-free setting; (2) UDOP~\cite{tang-etal-2022-udop}: multi-modal. In recent years, there has also been significant progress incorporating visual features into LLMs \citep{chen2023palix, mPLUG-owl2, gemini, chatgpt4}


% where the inputs are image-only 

For generative NLP tasks, like machine translation, performance on visually rich documents has not been explored in as much depth, though others have explored incorporating layout and visual features into machine translation. [13] examined including visual features into machine translation models in order to improve robustness to OCR errors in extracted text, leaving translation at the document level untouched. [17] looked at schema translation of tabular text which .....

In this work, we examine strategies for incorporating multi-modal information for document level translation of visually rich documents. We test the effectiveness of these strategies on a new benchmark a benchmark dataset that includes:

\bh{Maria: add a not about translation datasets here?}

\begin{itemize}
    \item LayoutLM~\citet{Xu2020LayoutLMPO}, XLayoutLM - using layout for information extraction. 
    \begin{itemize}
        \item FUNDS, XFUNDS datasets~\citep{xu-etal-2022-xfund} focus on NER. We have a more challenging dataset
        \item LoRaY - Multilingual dataset focus on text summarization task. We have a parallel dataset suitable for machine translation.
    \end{itemize}
    
    \item Doc2Doc - Documents are taken from WMT-newstest, TED, Europarl - ignores layout information.
    \item Doc2Sent - sliding windows, take from WMT, TED, Europarl - ignores layout
    
\end{itemize}

\paragraph{Datasets} For document-level machine translation evaluation,  publicly available evaluation datasets consist of plain text documents with sentence or paragraph level alignment. On such corpus is the JRC-Acquis which consists of 8,000 documents in 20 official EU languages which are automatically aligned at sentence and paragraph level \citep{steinberger-etal-2006-jrc}. Concurrent with this work, the Web Fiction benchmark\footnote{The Web Fiction corpus is released under a non-commercial license (CC-BY).} \citep{wang-EtAl:2023:WMT} was published consisting of entire web novel documents which were manually-aligned sentence pairs while preserving the book and chapter contexts. 



==> sections/5-analysis-ablation.tex <==
\section{Analysis}

